Exploring the Fairness and Resource Distribution in an Apache Mesos Environment

Apache Mesos, a cluster-wide resource manager, is widely deployed in massive scale at several Clouds and Data Centers. Mesos aims to provide high cluster utilization via fine grained resource co-scheduling and resource fairness among multiple users through Dominant Resource Fairness (DRF) based allocation. DRF takes into account different resource types (CPU, Memory, Disk I/O) requested by each application and determines the share of each cluster resource that could be allocated to the applications. Mesos has adopted a two-level scheduling policy: (1) DRF to allocate resources to competing frameworks and (2) task level scheduling by each framework for the resources allocated during the previous step. We have conducted experiments in a local Mesos cluster when used with frameworks such as Apache Aurora, Marathon, and our own framework Scylla, to study resource fairness and cluster utilization. Experimental results show how informed decision regarding second level scheduling policy of frameworks and attributes like offer holding period, offer refusal cycle and task arrival rate can reduce unfair resource distribution. Bin-Packing scheduling policy on Scylla with Marathon can reduce unfair allocation from 38\% to 3\%. By reducing unused free resources in offers we bring down the unfairness from to 90\% to 28\%. We also show the effect of task arrival rate to reduce the unfairness from 23\% to 7\%.

==> 3_Architecture.tex <==
\section{Architecture of Scylla with Apache Mesos and Docker Swarm}



==> 4_experimentalSetup.tex <==
\section{Experimental Setup}


==> 8_future_work.tex <==
\section{Future Work}

    

\begin{itemize}
\item{\textcolor{blue}{Random offer selection by allocation module:}
Apache Mesos resource allocation module picks an offer randomly and tries to assign it to the framework which has the lowest dominant share first. If the randomly selected offer is in the filter list, due to the refuse offer period, it will be assigned to the framework. If not, the resource will be offered to the next framework, which does not include the offer in the filter list. As Mesos Master does not make decisions based on the diverse demands of each framework, it can lead to wasteful allocation cycles. In a scenario where a large number of offers consists of resources such that it cannot launch any tasks. For example, an offer with the following resources \( <0 CPU, 0 GB memory, 1 MB disk>\) cannot launch any tasks which require CPU and memory resources. It will be intuitive to explore if the selection of offers can be made based on the demands of frameworks. This can be achieved by making changes to the allocation module of Mesos Master by implementing the callback functions for the allocation module \cite{ApacheModules} \cite{ApacheModulesb}.
}

\item {\textcolor{blue}{How fine-grained and coarse-grained allocation may effect:}
Apache Mesos allocation module allocate resource offers to frameworks based on their current dominant share. An offer can be rejected if not required by a framework or if not sufficient due to resource constraint. An accepted offer can be used by a framework in a fine grained mode where framework rescinds the extra resources so that this can be offered to other users. Some frameworks want to schedule tasks in a gang mode where available resources in offers are not sufficient. Frameworks can implement coarse-grained policy where it can hold resource offers from multiple cycle and wait till it accumulate enough to gang schedule all the tasks. This kind of gang scheduling and resource holding can cause dead lock situation and under utilization of resources in the cluster.  

}

\item {\textcolor{blue}{Expiring an offer by Mesos Master's allocation module:}
Mesos Master's allocation module allocates offers to frameworks based on the current dominant resource share of each frameowrk. Once assigned, a framework can either use those offers for launching tasks or can reject based on the requirement and the custom policy. Frameworks can hold an offer for launching tasks in future as per the framework policy. This can bring unfair distribution as other users with lower dominant share may starve for resources. Mesos Masters can set an offer timeout duration before which an offer is rescinded from a framework even though a framework wants to hold the offer. If the offer expiry period is not set then a framework can hold an offer as long as it wants. Depending upon cluster's need and policy of other frameworks, an altered offer expiry period can be utilized wisely for better resource distribution. 
}
\item {\textcolor{blue}{Mesos master penalize frameworks for not using offers}}
\end{itemize}


